Have we been Naive to Select Machine Learning Models? Noisy Data are here to Stay!

The model selection procedure is usually a single-criterion decision making in which we select the model that maximizes a specific metric in a specific set, such as the Validation set performance. We claim this is very naive and can perform poor selections of over-fitted models due to the over-searching phenomenon, which over-estimates the performance on that specific set. Futhermore, real world data contains noise that should not be ignored by the model selection procedure and must be taken into account when performing model selection. Also, we have defined four theoretical optimality conditions that we can pursue to better select the models and analyze them by using a multi-criteria decision-making algorithm (TOPSIS) that considers proxies to the optimality conditions to select reasonable models.

==> figures/reduced_statistical_low_complexity_processed.tex <==
\begin{table}
\centering
\label{tab:reduced_statistical_low_complexity}
\begin{tabular}{lllllllr}
\toprule
{} &              TTVH &             TTVHN &              THT &              THTN &             TTVHT &            TTVHTN &  Summary Test Acc \\
Policy &                   &                   &                  &                   &                   &                   &                   \\
\midrule
TTVH   &          $\equiv$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &                -3 \\
TTVHN  &   $\triangledown$ &          $\equiv$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &                -5 \\
THT    &  $\blacktriangle$ &  $\blacktriangle$ &         $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &                 5 \\
THTN   &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &                 1 \\
TTVHT  &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &                 3 \\
TTVHTN &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &                -1 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/low_complexity_processed.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cc|c|c|cccc|ccc}
\toprule
 \multicolumn{2}{c|}{\multirow{2}{*}{Policy}}& \multirow{2}{*}{\# Neurons $\downarrow$}   & \multirow{2}{*}{\# Epochs $\uparrow$} &\multicolumn{4}{c|}{Accuracy $\uparrow$} & \multicolumn{3}{c}{Disagreement $\downarrow$} \\
              &      &     &   &        Train &   Validation &      Holdout &         Test & Train-Validation & Holdout-Test &         All \\
\midrule
\multirow{9}{*}{Individual} & TTVH &  \makecell{75.98\\(27.06)} &  \makecell{82.64\\(26.28)} &    \makecell{91.49\\(8.4)} &   \makecell{91.1\\(7.09)} &   \makecell{91.5\\(7.91)} &   \makecell{85.42\\(9.39)} &      \makecell{2.26\\(2.36)} &  \makecell{6.26\\(6.91)} &  \makecell{3.84\\(3.59)} \\
       & TTVHN &   \makecell{10.27\\(9.27)} &   \makecell{78.08\\(28.3)} &   \makecell{87.59\\(7.94)} &  \makecell{88.36\\(7.13)} &  \makecell{87.83\\(7.66)} &    \makecell{82.9\\(9.96)} &      \makecell{2.14\\(1.93)} &  \makecell{5.54\\(7.19)} &  \makecell{3.54\\(3.74)} \\
       & THT &   \makecell{75.5\\(24.61)} &  \makecell{78.21\\(27.19)} &   \makecell{91.22\\(8.36)} &  \makecell{89.05\\(7.89)} &   \makecell{90.9\\(8.07)} &   \makecell{89.65\\(7.34)} &      \makecell{2.83\\(2.67)} &  \makecell{3.52\\(3.26)} &   \makecell{2.67\\(2.0)} \\
       & THTN &    \makecell{8.75\\(7.24)} &   \makecell{78.35\\(27.0)} &   \makecell{86.78\\(7.93)} &  \makecell{85.97\\(8.22)} &    \makecell{86.7\\(7.8)} &    \makecell{86.9\\(7.94)} &      \makecell{2.37\\(2.65)} &  \makecell{2.75\\(2.11)} &    \makecell{2.2\\(1.6)} \\
       & TTVHT &   \makecell{76.5\\(24.32)} &  \makecell{77.75\\(27.45)} &    \makecell{91.05\\(8.5)} &  \makecell{90.47\\(7.21)} &   \makecell{91.05\\(8.0)} &   \makecell{88.88\\(7.78)} &      \makecell{2.52\\(2.45)} &  \makecell{3.42\\(3.53)} &  \makecell{2.48\\(2.11)} \\
       & TTVHTN &   \makecell{11.37\\(9.44)} &  \makecell{77.48\\(27.79)} &   \makecell{87.54\\(7.92)} &  \makecell{88.14\\(7.13)} &  \makecell{87.76\\(7.61)} &   \makecell{86.44\\(8.35)} &      \makecell{2.09\\(1.93)} &  \makecell{3.15\\(3.58)} &   \makecell{2.3\\(1.93)} \\
\midrule
\multirow{9}{*}{Local} & TTVH &  \makecell{88.13\\(14.07)} &  \makecell{75.85\\(27.77)} &    \makecell{90.9\\(8.51)} &  \makecell{90.36\\(7.27)} &  \makecell{90.93\\(7.99)} &   \makecell{85.51\\(9.29)} &      \makecell{2.43\\(2.34)} &  \makecell{5.71\\(6.44)} &  \makecell{3.62\\(3.43)} \\
       & TTVHN &   \makecell{15.97\\(8.89)} &  \makecell{77.12\\(27.25)} &    \makecell{87.76\\(7.9)} &   \makecell{88.0\\(7.32)} &    \makecell{87.9\\(7.6)} &  \makecell{83.33\\(10.02)} &      \makecell{2.22\\(2.24)} &  \makecell{5.23\\(6.55)} &  \makecell{3.39\\(3.43)} \\
       & THT &  \makecell{82.75\\(19.23)} &  \makecell{68.67\\(30.14)} &   \makecell{90.56\\(8.51)} &  \makecell{88.58\\(7.57)} &  \makecell{90.28\\(8.03)} &   \makecell{88.76\\(7.59)} &      \makecell{3.26\\(3.32)} &  \makecell{3.58\\(3.79)} &   \makecell{2.86\\(2.4)} \\
       & THTN &   \makecell{13.13\\(7.47)} &  \makecell{74.71\\(26.79)} &   \makecell{86.77\\(8.84)} &  \makecell{85.91\\(8.06)} &    \makecell{86.8\\(7.9)} &   \makecell{86.26\\(8.27)} &      \makecell{2.53\\(3.83)} &  \makecell{3.15\\(2.98)} &  \makecell{2.42\\(2.34)} \\
       & TTVHT &   \makecell{85.79\\(16.7)} &  \makecell{68.76\\(30.63)} &   \makecell{90.51\\(8.55)} &  \makecell{89.58\\(7.33)} &  \makecell{90.45\\(8.02)} &    \makecell{87.85\\(8.1)} &      \makecell{2.88\\(2.77)} &   \makecell{3.7\\(4.36)} &  \makecell{2.78\\(2.54)} \\
       & TTVHTN &   \makecell{17.63\\(10.1)} &  \makecell{77.45\\(26.62)} &   \makecell{87.81\\(8.17)} &   \makecell{87.62\\(7.3)} &   \makecell{87.9\\(7.66)} &   \makecell{85.84\\(8.53)} &      \makecell{2.51\\(2.68)} &  \makecell{3.48\\(4.24)} &  \makecell{2.59\\(2.45)} \\
\midrule
\multirow{9}{*}{Global} & TTVH &   \makecell{92.86\\(10.0)} &  \makecell{72.07\\(28.75)} &   \makecell{90.68\\(8.25)} &  \makecell{89.82\\(7.55)} &  \makecell{90.58\\(7.96)} &   \makecell{85.31\\(9.36)} &      \makecell{2.39\\(2.25)} &  \makecell{5.64\\(7.08)} &  \makecell{3.57\\(3.77)} \\
       & TTVHN &  \makecell{19.21\\(10.13)} &  \makecell{76.32\\(26.87)} &   \makecell{87.52\\(8.04)} &  \makecell{87.66\\(7.64)} &  \makecell{87.64\\(7.74)} &  \makecell{83.21\\(10.24)} &      \makecell{2.12\\(2.13)} &  \makecell{4.99\\(6.82)} &  \makecell{3.23\\(3.62)} \\
       & THT &  \makecell{89.36\\(12.43)} &  \makecell{69.11\\(30.22)} &  \makecell{90.04\\(10.02)} &  \makecell{88.45\\(7.74)} &   \makecell{90.21\\(8.2)} &   \makecell{87.44\\(8.42)} &      \makecell{3.59\\(3.66)} &    \makecell{3.9\\(4.9)} &   \makecell{3.18\\(2.9)} \\
       & THTN &   \makecell{13.36\\(6.87)} &  \makecell{71.53\\(27.49)} &   \makecell{86.09\\(9.84)} &   \makecell{85.7\\(8.39)} &  \makecell{86.62\\(7.89)} &    \makecell{85.08\\(9.0)} &      \makecell{2.95\\(4.19)} &   \makecell{3.4\\(4.15)} &  \makecell{2.75\\(2.83)} \\
       & TTVHT &   \makecell{94.86\\(5.01)} &  \makecell{68.78\\(30.02)} &    \makecell{90.45\\(8.4)} &   \makecell{89.31\\(7.5)} &  \makecell{90.28\\(8.01)} &   \makecell{86.94\\(8.51)} &      \makecell{2.67\\(2.73)} &  \makecell{4.12\\(5.11)} &   \makecell{2.9\\(2.89)} \\
       & TTVHTN &  \makecell{20.93\\(13.45)} &  \makecell{76.09\\(25.73)} &    \makecell{87.67\\(8.1)} &  \makecell{87.42\\(7.62)} &  \makecell{87.73\\(7.74)} &    \makecell{85.37\\(8.8)} &      \makecell{2.21\\(2.41)} &  \makecell{3.86\\(4.75)} &  \makecell{2.66\\(2.64)} \\
\bottomrule
\end{tabular}
}
\caption{Low Complexity Results}
\label{tab:low_complexity}
\end{table}


==> tables/no_premature_early_stopping_processed.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllllll}
\toprule
       &         &   Architecture & Early Stopping & \multicolumn{4}{l}{Accuracy} & \multicolumn{3}{l}{Disagreement} \\
       &         &      \# Neurons &       \# Epochs &          Train &    Validation &       Holdout &           Test & Train-Validation & Holdout-Test &          All \\
(Selection Strategy, Group) & (Selection Strategy, Policy) &                &                &                &               &               &                &                  &              &              \\
\midrule
Individual & TTVHN &   \makecell{10.27\\(9.27)} &   \makecell{78.08\\(28.3)} &   \makecell{87.59\\(7.94)} &  \makecell{88.36\\(7.13)} &  \makecell{87.83\\(7.66)} &    \makecell{82.9\\(9.96)} &      \makecell{2.14\\(1.93)} &  \makecell{5.54\\(7.19)} &  \makecell{3.54\\(3.74)} \\
       & TTVHNB &   \makecell{13.8\\(12.23)} &  \makecell{17.94\\(20.68)} &   \makecell{83.41\\(7.61)} &  \makecell{85.37\\(7.33)} &  \makecell{84.01\\(7.38)} &  \makecell{80.48\\(10.26)} &      \makecell{2.68\\(2.17)} &  \makecell{4.63\\(5.87)} &  \makecell{3.34\\(3.24)} \\
       & TTVHNE &   \makecell{10.77\\(9.38)} &  \makecell{89.83\\(24.46)} &   \makecell{87.53\\(7.96)} &  \makecell{87.79\\(7.08)} &  \makecell{87.66\\(7.66)} &   \makecell{82.96\\(9.91)} &       \makecell{2.2\\(2.06)} &  \makecell{5.33\\(6.87)} &  \makecell{3.41\\(3.64)} \\
       & THTN &    \makecell{8.75\\(7.24)} &   \makecell{78.35\\(27.0)} &   \makecell{86.78\\(7.93)} &  \makecell{85.97\\(8.22)} &    \makecell{86.7\\(7.8)} &    \makecell{86.9\\(7.94)} &      \makecell{2.37\\(2.65)} &  \makecell{2.75\\(2.11)} &    \makecell{2.2\\(1.6)} \\
       & THTNB &   \makecell{11.17\\(8.83)} &   \makecell{16.53\\(20.6)} &   \makecell{81.83\\(8.28)} &  \makecell{83.49\\(8.61)} &  \makecell{82.49\\(8.14)} &   \makecell{82.63\\(9.74)} &       \makecell{2.39\\(2.7)} &  \makecell{3.08\\(3.03)} &  \makecell{2.44\\(2.04)} \\
       & THTNE &     \makecell{8.49\\(6.9)} &  \makecell{89.79\\(24.18)} &   \makecell{86.69\\(8.26)} &  \makecell{85.53\\(8.19)} &  \makecell{86.61\\(7.89)} &   \makecell{86.14\\(8.12)} &      \makecell{2.53\\(2.84)} &  \makecell{2.62\\(2.69)} &  \makecell{2.19\\(1.88)} \\
       & TTVHTN &   \makecell{11.37\\(9.44)} &  \makecell{77.48\\(27.79)} &   \makecell{87.54\\(7.92)} &  \makecell{88.14\\(7.13)} &  \makecell{87.76\\(7.61)} &   \makecell{86.44\\(8.35)} &      \makecell{2.09\\(1.93)} &  \makecell{3.15\\(3.58)} &   \makecell{2.3\\(1.93)} \\
       & TTVHTNE &  \makecell{11.89\\(10.47)} &  \makecell{89.55\\(24.41)} &   \makecell{87.53\\(7.93)} &  \makecell{87.85\\(7.19)} &   \makecell{87.7\\(7.66)} &     \makecell{85.9\\(8.3)} &      \makecell{2.04\\(2.11)} &  \makecell{3.39\\(4.05)} &  \makecell{2.39\\(2.23)} \\
       & TTVHTNB &  \makecell{14.91\\(12.97)} &  \makecell{19.09\\(21.61)} &   \makecell{83.78\\(7.08)} &   \makecell{85.7\\(6.92)} &  \makecell{84.38\\(6.89)} &   \makecell{83.37\\(8.09)} &       \makecell{2.59\\(2.4)} &   \makecell{3.3\\(3.41)} &  \makecell{2.62\\(2.04)} \\
Local & TTVHN &   \makecell{15.97\\(8.89)} &  \makecell{77.12\\(27.25)} &    \makecell{87.76\\(7.9)} &   \makecell{88.0\\(7.32)} &    \makecell{87.9\\(7.6)} &  \makecell{83.33\\(10.02)} &      \makecell{2.22\\(2.24)} &  \makecell{5.23\\(6.55)} &  \makecell{3.39\\(3.43)} \\
       & TTVHNB &  \makecell{23.77\\(13.85)} &  \makecell{22.58\\(22.84)} &   \makecell{83.83\\(8.09)} &  \makecell{85.58\\(7.37)} &  \makecell{84.66\\(7.18)} &   \makecell{80.73\\(9.69)} &      \makecell{2.78\\(3.07)} &  \makecell{4.77\\(6.13)} &  \makecell{3.43\\(3.34)} \\
       & TTVHNE &   \makecell{16.26\\(9.87)} &   \makecell{88.5\\(24.45)} &   \makecell{87.55\\(8.01)} &  \makecell{87.22\\(7.31)} &   \makecell{87.57\\(7.6)} &   \makecell{83.29\\(9.78)} &       \makecell{2.4\\(2.53)} &    \makecell{5.1\\(6.5)} &   \makecell{3.33\\(3.5)} \\
       & THTN &   \makecell{13.13\\(7.47)} &  \makecell{74.71\\(26.79)} &   \makecell{86.77\\(8.84)} &  \makecell{85.91\\(8.06)} &    \makecell{86.8\\(7.9)} &   \makecell{86.26\\(8.27)} &      \makecell{2.53\\(3.83)} &  \makecell{3.15\\(2.98)} &  \makecell{2.42\\(2.34)} \\
       & THTNB &  \makecell{19.75\\(11.53)} &   \makecell{21.6\\(23.26)} &  \makecell{81.97\\(10.99)} &  \makecell{83.99\\(8.16)} &   \makecell{83.5\\(7.59)} &    \makecell{82.04\\(9.3)} &       \makecell{3.45\\(6.3)} &  \makecell{3.41\\(4.37)} &  \makecell{3.06\\(3.71)} \\
       & THTNE &   \makecell{12.98\\(8.03)} &  \makecell{88.87\\(24.11)} &  \makecell{86.21\\(10.19)} &   \makecell{85.5\\(8.02)} &  \makecell{86.66\\(7.86)} &    \makecell{85.0\\(8.71)} &      \makecell{3.35\\(4.93)} &  \makecell{3.36\\(4.27)} &  \makecell{2.86\\(3.18)} \\
       & TTVHTN &   \makecell{17.63\\(10.1)} &  \makecell{77.45\\(26.62)} &   \makecell{87.81\\(8.17)} &   \makecell{87.62\\(7.3)} &   \makecell{87.9\\(7.66)} &   \makecell{85.84\\(8.53)} &      \makecell{2.51\\(2.68)} &  \makecell{3.48\\(4.24)} &  \makecell{2.59\\(2.45)} \\
       & TTVHTNE &   \makecell{17.27\\(10.0)} &  \makecell{87.87\\(24.53)} &   \makecell{87.68\\(8.13)} &  \makecell{87.23\\(7.34)} &  \makecell{87.67\\(7.71)} &   \makecell{85.27\\(8.46)} &      \makecell{2.59\\(2.61)} &  \makecell{3.72\\(4.59)} &  \makecell{2.72\\(2.62)} \\
       & TTVHTNB &  \makecell{25.49\\(14.51)} &  \makecell{24.77\\(23.23)} &   \makecell{84.51\\(7.99)} &  \makecell{86.15\\(7.02)} &  \makecell{85.31\\(6.95)} &   \makecell{83.09\\(8.25)} &      \makecell{2.92\\(3.18)} &  \makecell{3.95\\(4.96)} &  \makecell{3.03\\(2.94)} \\
Global & TTVHN &  \makecell{19.21\\(10.13)} &  \makecell{76.32\\(26.87)} &   \makecell{87.52\\(8.04)} &  \makecell{87.66\\(7.64)} &  \makecell{87.64\\(7.74)} &  \makecell{83.21\\(10.24)} &      \makecell{2.12\\(2.13)} &  \makecell{4.99\\(6.82)} &  \makecell{3.23\\(3.62)} \\
       & TTVHNB &  \makecell{25.79\\(12.75)} &  \makecell{25.81\\(26.57)} &   \makecell{84.59\\(7.12)} &  \makecell{85.66\\(7.28)} &  \makecell{85.01\\(6.96)} &   \makecell{81.23\\(8.65)} &      \makecell{2.31\\(2.52)} &    \makecell{4.6\\(6.7)} &  \makecell{3.12\\(3.64)} \\
       & TTVHNE &  \makecell{18.57\\(12.03)} &  \makecell{86.83\\(24.43)} &    \makecell{87.4\\(8.27)} &  \makecell{86.59\\(7.57)} &  \makecell{87.35\\(7.79)} &    \makecell{82.9\\(10.5)} &      \makecell{2.34\\(2.54)} &  \makecell{5.05\\(7.23)} &  \makecell{3.31\\(3.91)} \\
       & THTN &   \makecell{13.36\\(6.87)} &  \makecell{71.53\\(27.49)} &   \makecell{86.09\\(9.84)} &   \makecell{85.7\\(8.39)} &  \makecell{86.62\\(7.89)} &    \makecell{85.08\\(9.0)} &      \makecell{2.95\\(4.19)} &   \makecell{3.4\\(4.15)} &  \makecell{2.75\\(2.83)} \\
       & THTNB &   \makecell{23.93\\(9.36)} &    \makecell{25.5\\(27.5)} &  \makecell{82.87\\(10.05)} &  \makecell{84.43\\(7.75)} &   \makecell{84.1\\(7.07)} &   \makecell{82.17\\(8.44)} &      \makecell{3.19\\(5.78)} &  \makecell{3.72\\(4.78)} &  \makecell{3.08\\(3.66)} \\
       & THTNE &    \makecell{11.5\\(8.06)} &  \makecell{86.83\\(23.81)} &   \makecell{85.77\\(9.33)} &  \makecell{84.99\\(8.07)} &  \makecell{86.17\\(7.53)} &   \makecell{83.89\\(9.03)} &      \makecell{3.22\\(4.17)} &  \makecell{3.61\\(4.91)} &  \makecell{2.91\\(3.13)} \\
       & TTVHTN &  \makecell{20.93\\(13.45)} &  \makecell{76.09\\(25.73)} &    \makecell{87.67\\(8.1)} &  \makecell{87.42\\(7.62)} &  \makecell{87.73\\(7.74)} &    \makecell{85.37\\(8.8)} &      \makecell{2.21\\(2.41)} &  \makecell{3.86\\(4.75)} &  \makecell{2.66\\(2.64)} \\
       & TTVHTNE &  \makecell{20.57\\(13.45)} &   \makecell{86.5\\(24.03)} &   \makecell{87.68\\(8.24)} &  \makecell{86.57\\(7.65)} &   \makecell{87.58\\(7.8)} &    \makecell{84.4\\(9.17)} &      \makecell{2.47\\(2.76)} &  \makecell{4.12\\(5.35)} &  \makecell{2.85\\(2.98)} \\
       & TTVHTNB &  \makecell{28.79\\(14.76)} &  \makecell{29.16\\(24.88)} &    \makecell{85.43\\(7.4)} &   \makecell{86.4\\(7.39)} &  \makecell{85.85\\(7.14)} &   \makecell{83.13\\(8.68)} &       \makecell{2.46\\(2.3)} &  \makecell{3.99\\(5.74)} &  \makecell{2.87\\(3.09)} \\
\bottomrule
\end{tabular}
}
\caption{No Premature Early Stopping Results}
\label{tab:no_premature_early_stopping}
\end{table}


==> tables/policy_sbss_no_sbss.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrrrrrr}
\toprule
{} & \multicolumn{4}{l}{SBSS} & \multicolumn{4}{l}{Stratified 10-fold} \\
Accuracy & Train & Validation & Holdout &  Test &              Train & Validation & Holdout &  Test \\
Policy     &       &            &         &       &                    &            &         &       \\
\midrule
Oracle     &  0.87 &       0.87 &    0.88 &  0.91 &               0.80 &       0.82 &    0.82 &  0.87 \\
Holdout    &  0.92 &       0.90 &    0.92 &  0.86 &               0.83 &       0.85 &    0.86 &  0.81 \\
Train      &  0.92 &       0.87 &    0.91 &  0.85 &               0.86 &       0.82 &    0.84 &  0.81 \\
Validation &  0.88 &       0.92 &    0.89 &  0.84 &               0.81 &       0.88 &    0.84 &  0.80 \\
\bottomrule
\end{tabular}
\caption{SBSS}
\label{tab:policy_sbss_no_sbss.tex}
\end{table}


==> tables/similar_sets_performance_processed.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cc|c|c|cccc|ccc}
\toprule
 \multicolumn{2}{c|}{\multirow{2}{*}{Policy}}& \multirow{2}{*}{\# Neurons $\downarrow$}   & \multirow{2}{*}{\# Epochs $\uparrow$} &\multicolumn{4}{c|}{Accuracy $\uparrow$} & \multicolumn{3}{c}{Disagreement $\downarrow$} \\
              &      &     &   &        Train &   Validation &      Holdout &         Test & Train-Validation & Holdout-Test &         All \\
\midrule
%         \multirow{9}{*}{Individual} & Holdout &  \makecell{76.41\\(27.5)} &  \makecell{84.79\\(25.13)} &  \makecell{92.08\\(7.92)} & \makecell{89.94\\(7.79)} & \makecell{91.76\\(7.66)} & \makecell{85.54\\(9.29)} &      \makecell{2.77\\(2.66)} &  \makecell{6.37\\(6.53)} & \makecell{3.94\\(3.51)} \\
%          &    Test &  \makecell{42.8\\(33.91)} &  \makecell{63.72\\(34.72)} &   \makecell{87.42\\(8.8)} & \makecell{87.07\\(7.64)} & \makecell{87.68\\(7.98)} & \makecell{90.61\\(7.05)} &      \makecell{2.67\\(3.25)} &  \makecell{4.29\\(3.51)} & \makecell{3.13\\(2.41)} \\
%          &     THT &  \makecell{75.5\\(24.61)} &  \makecell{78.21\\(27.19)} &  \makecell{91.22\\(8.36)} & \makecell{89.05\\(7.89)} &  \makecell{90.9\\(8.07)} & \makecell{89.65\\(7.34)} &      \makecell{2.83\\(2.67)} &  \makecell{3.52\\(3.26)} &  \makecell{2.67\\(2.0)} \\
%          &    TTVH & \makecell{75.98\\(27.06)} &  \makecell{82.64\\(26.28)} &   \makecell{91.49\\(8.4)} &  \makecell{91.1\\(7.09)} &  \makecell{91.5\\(7.91)} & \makecell{85.42\\(9.39)} &      \makecell{2.26\\(2.36)} &  \makecell{6.26\\(6.91)} & \makecell{3.84\\(3.59)} \\
%          &   TTVHT &  \makecell{76.5\\(24.32)} &  \makecell{77.75\\(27.45)} &   \makecell{91.05\\(8.5)} & \makecell{90.47\\(7.21)} &  \makecell{91.05\\(8.0)} & \makecell{88.88\\(7.78)} &      \makecell{2.52\\(2.45)} &  \makecell{3.42\\(3.53)} & \makecell{2.48\\(2.11)} \\
% \midrule
%              \multirow{9}{*}{Local} & Holdout &  \makecell{86.41\\(17.5)} &  \makecell{78.35\\(27.47)} &  \makecell{91.52\\(8.01)} &  \makecell{89.37\\(7.6)} &  \makecell{91.2\\(7.71)} &  \makecell{85.01\\(9.6)} &      \makecell{2.76\\(2.76)} &  \makecell{6.36\\(7.27)} & \makecell{3.94\\(3.97)} \\
%               &    Test & \makecell{68.52\\(30.98)} &   \makecell{61.08\\(34.2)} &  \makecell{88.61\\(9.19)} & \makecell{88.13\\(7.81)} & \makecell{88.77\\(8.51)} & \makecell{89.05\\(7.49)} &      \makecell{2.28\\(2.62)} &  \makecell{3.46\\(3.28)} & \makecell{2.48\\(2.11)} \\
%               &     THT & \makecell{82.75\\(19.23)} &  \makecell{68.67\\(30.14)} &  \makecell{90.56\\(8.51)} & \makecell{88.58\\(7.57)} & \makecell{90.28\\(8.03)} & \makecell{88.76\\(7.59)} &      \makecell{3.26\\(3.32)} &  \makecell{3.58\\(3.79)} &  \makecell{2.86\\(2.4)} \\
%               &    TTVH & \makecell{88.13\\(14.07)} &  \makecell{75.85\\(27.77)} &   \makecell{90.9\\(8.51)} & \makecell{90.36\\(7.27)} & \makecell{90.93\\(7.99)} & \makecell{85.51\\(9.29)} &      \makecell{2.43\\(2.34)} &  \makecell{5.71\\(6.44)} & \makecell{3.62\\(3.43)} \\
%               &   TTVHT &  \makecell{85.79\\(16.7)} &  \makecell{68.76\\(30.63)} &  \makecell{90.51\\(8.55)} & \makecell{89.58\\(7.33)} & \makecell{90.45\\(8.02)} &  \makecell{87.85\\(8.1)} &      \makecell{2.88\\(2.77)} &   \makecell{3.7\\(4.36)} & \makecell{2.78\\(2.54)} \\
% \midrule
%             \multirow{9}{*}{Global} & Holdout & \makecell{87.36\\(23.97)} &  \makecell{75.85\\(26.96)} &  \makecell{90.99\\(8.93)} & \makecell{88.78\\(7.87)} & \makecell{90.83\\(8.02)} & \makecell{85.48\\(9.18)} &      \makecell{3.08\\(2.75)} &  \makecell{5.49\\(6.39)} & \makecell{3.67\\(3.47)} \\
%              &    Test &  \makecell{85.0\\(21.18)} &   \makecell{62.13\\(32.4)} &  \makecell{89.37\\(8.82)} & \makecell{88.26\\(8.03)} & \makecell{89.24\\(8.46)} & \makecell{87.69\\(8.17)} &      \makecell{2.24\\(3.15)} &    \makecell{3.4\\(4.4)} & \makecell{2.42\\(2.74)} \\
%              &     THT & \makecell{89.36\\(12.43)} &  \makecell{69.11\\(30.22)} & \makecell{90.04\\(10.02)} & \makecell{88.45\\(7.74)} &  \makecell{90.21\\(8.2)} & \makecell{87.44\\(8.42)} &      \makecell{3.59\\(3.66)} &    \makecell{3.9\\(4.9)} &  \makecell{3.18\\(2.9)} \\
%              &    TTVH &  \makecell{92.86\\(10.0)} &  \makecell{72.07\\(28.75)} &  \makecell{90.68\\(8.25)} & \makecell{89.82\\(7.55)} & \makecell{90.58\\(7.96)} & \makecell{85.31\\(9.36)} &      \makecell{2.39\\(2.25)} &  \makecell{5.64\\(7.08)} & \makecell{3.57\\(3.77)} \\
%              &   TTVHT &  \makecell{94.86\\(5.01)} &  \makecell{68.78\\(30.02)} &   \makecell{90.45\\(8.4)} &  \makecell{89.31\\(7.5)} & \makecell{90.28\\(8.01)} & \makecell{86.94\\(8.51)} &      \makecell{2.67\\(2.73)} &  \makecell{4.12\\(5.11)} &  \makecell{2.9\\(2.89)} \\
\multirow{9}{*}{Individual} & Holdout &   \makecell{76.41\\(27.5)} &  \makecell{84.79\\(25.13)} &   \makecell{92.08\\(7.92)} &  \makecell{89.94\\(7.79)} &  \makecell{91.76\\(7.66)} &  \makecell{85.54\\(9.29)} &      \makecell{2.77\\(2.66)} &  \makecell{6.37\\(6.53)} &  \makecell{3.94\\(3.51)} \\
       & TTVH &  \makecell{75.98\\(27.06)} &  \makecell{82.64\\(26.28)} &    \makecell{91.49\\(8.4)} &   \makecell{91.1\\(7.09)} &   \makecell{91.5\\(7.91)} &  \makecell{85.42\\(9.39)} &      \makecell{2.26\\(2.36)} &  \makecell{6.26\\(6.91)} &  \makecell{3.84\\(3.59)} \\
       & Test &   \makecell{42.8\\(33.91)} &  \makecell{63.72\\(34.72)} &    \makecell{87.42\\(8.8)} &  \makecell{87.07\\(7.64)} &  \makecell{87.68\\(7.98)} &  \makecell{90.61\\(7.05)} &      \makecell{2.67\\(3.25)} &  \makecell{4.29\\(3.51)} &  \makecell{3.13\\(2.41)} \\
       & THT &   \makecell{75.5\\(24.61)} &  \makecell{78.21\\(27.19)} &   \makecell{91.22\\(8.36)} &  \makecell{89.05\\(7.89)} &   \makecell{90.9\\(8.07)} &  \makecell{89.65\\(7.34)} &      \makecell{2.83\\(2.67)} &  \makecell{3.52\\(3.26)} &   \makecell{2.67\\(2.0)} \\
       & TTVHT &   \makecell{76.5\\(24.32)} &  \makecell{77.75\\(27.45)} &    \makecell{91.05\\(8.5)} &  \makecell{90.47\\(7.21)} &   \makecell{91.05\\(8.0)} &  \makecell{88.88\\(7.78)} &      \makecell{2.52\\(2.45)} &  \makecell{3.42\\(3.53)} &  \makecell{2.48\\(2.11)} \\
\midrule
\multirow{9}{*}{Local} & Holdout &   \makecell{86.41\\(17.5)} &  \makecell{78.35\\(27.47)} &   \makecell{91.52\\(8.01)} &   \makecell{89.37\\(7.6)} &   \makecell{91.2\\(7.71)} &   \makecell{85.01\\(9.6)} &      \makecell{2.76\\(2.76)} &  \makecell{6.36\\(7.27)} &  \makecell{3.94\\(3.97)} \\
       & TTVH &  \makecell{88.13\\(14.07)} &  \makecell{75.85\\(27.77)} &    \makecell{90.9\\(8.51)} &  \makecell{90.36\\(7.27)} &  \makecell{90.93\\(7.99)} &  \makecell{85.51\\(9.29)} &      \makecell{2.43\\(2.34)} &  \makecell{5.71\\(6.44)} &  \makecell{3.62\\(3.43)} \\
       & Test &  \makecell{68.52\\(30.98)} &   \makecell{61.08\\(34.2)} &   \makecell{88.61\\(9.19)} &  \makecell{88.13\\(7.81)} &  \makecell{88.77\\(8.51)} &  \makecell{89.05\\(7.49)} &      \makecell{2.28\\(2.62)} &  \makecell{3.46\\(3.28)} &  \makecell{2.48\\(2.11)} \\
       & THT &  \makecell{82.75\\(19.23)} &  \makecell{68.67\\(30.14)} &   \makecell{90.56\\(8.51)} &  \makecell{88.58\\(7.57)} &  \makecell{90.28\\(8.03)} &  \makecell{88.76\\(7.59)} &      \makecell{3.26\\(3.32)} &  \makecell{3.58\\(3.79)} &   \makecell{2.86\\(2.4)} \\
       & TTVHT &   \makecell{85.79\\(16.7)} &  \makecell{68.76\\(30.63)} &   \makecell{90.51\\(8.55)} &  \makecell{89.58\\(7.33)} &  \makecell{90.45\\(8.02)} &   \makecell{87.85\\(8.1)} &      \makecell{2.88\\(2.77)} &   \makecell{3.7\\(4.36)} &  \makecell{2.78\\(2.54)} \\
\midrule
\multirow{9}{*}{Global} & Holdout &  \makecell{87.36\\(23.97)} &  \makecell{75.85\\(26.96)} &   \makecell{90.99\\(8.93)} &  \makecell{88.78\\(7.87)} &  \makecell{90.83\\(8.02)} &  \makecell{85.48\\(9.18)} &      \makecell{3.08\\(2.75)} &  \makecell{5.49\\(6.39)} &  \makecell{3.67\\(3.47)} \\
       & TTVH &   \makecell{92.86\\(10.0)} &  \makecell{72.07\\(28.75)} &   \makecell{90.68\\(8.25)} &  \makecell{89.82\\(7.55)} &  \makecell{90.58\\(7.96)} &  \makecell{85.31\\(9.36)} &      \makecell{2.39\\(2.25)} &  \makecell{5.64\\(7.08)} &  \makecell{3.57\\(3.77)} \\
       & Test &   \makecell{85.0\\(21.18)} &   \makecell{62.13\\(32.4)} &   \makecell{89.37\\(8.82)} &  \makecell{88.26\\(8.03)} &  \makecell{89.24\\(8.46)} &  \makecell{87.69\\(8.17)} &      \makecell{2.24\\(3.15)} &    \makecell{3.4\\(4.4)} &  \makecell{2.42\\(2.74)} \\
       & THT &  \makecell{89.36\\(12.43)} &  \makecell{69.11\\(30.22)} &  \makecell{90.04\\(10.02)} &  \makecell{88.45\\(7.74)} &   \makecell{90.21\\(8.2)} &  \makecell{87.44\\(8.42)} &      \makecell{3.59\\(3.66)} &    \makecell{3.9\\(4.9)} &   \makecell{3.18\\(2.9)} \\
       & TTVHT &   \makecell{94.86\\(5.01)} &  \makecell{68.78\\(30.02)} &    \makecell{90.45\\(8.4)} &   \makecell{89.31\\(7.5)} &  \makecell{90.28\\(8.01)} &  \makecell{86.94\\(8.51)} &      \makecell{2.67\\(2.73)} &  \makecell{4.12\\(5.11)} &   \makecell{2.9\\(2.89)} \\
\bottomrule
\end{tabular}
}
\caption{Results for High Robustness policies.}
\label{tab:similar_sets_performance}
\end{table}


==> tables/single_sets_processed.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cc|c|c|cccc|ccc}
\toprule
 \multicolumn{2}{c|}{\multirow{2}{*}{Policy}}& \multirow{2}{*}{\# Neurons}   & \multirow{2}{*}{\# Epochs} &\multicolumn{4}{c|}{Accuracy} & \multicolumn{3}{c}{Disagreement} \\
              &      &     &   &        Train &   Validation &      Holdout &         Test & Train-Validation & Holdout-Test &         All \\
\midrule
                        \multirow{7}{*}{Individual} &      Train & \makecell{73.47\\(29.13)} &   \makecell{86.02\\(24.6)} & \makecell{92.45\\(7.72)} &  \makecell{87.47\\(7.8)} & \makecell{91.28\\(7.71)} &  \makecell{85.06\\(9.5)} &      \makecell{5.03\\(4.21)} &   \makecell{6.4\\(6.84)} & \makecell{4.66\\(4.05)} \\
         & Validation & \makecell{47.02\\(34.84)} &  \makecell{62.99\\(35.21)} &  \makecell{87.85\\(8.8)} & \makecell{91.86\\(6.85)} & \makecell{88.97\\(7.98)} & \makecell{84.25\\(9.78)} &      \makecell{4.26\\(3.96)} &  \makecell{5.21\\(6.76)} & \makecell{4.38\\(3.83)} \\
         &    Holdout &  \makecell{76.41\\(27.5)} &  \makecell{84.79\\(25.13)} & \makecell{92.08\\(7.92)} & \makecell{89.94\\(7.79)} & \makecell{91.76\\(7.66)} & \makecell{85.54\\(9.29)} &      \makecell{2.77\\(2.66)} &  \makecell{6.37\\(6.53)} & \makecell{3.94\\(3.51)} \\
         &       Test &  \makecell{42.8\\(33.91)} &  \makecell{63.72\\(34.72)} &  \makecell{87.42\\(8.8)} & \makecell{87.07\\(7.64)} & \makecell{87.68\\(7.98)} & \makecell{90.61\\(7.05)} &      \makecell{2.67\\(3.25)} &  \makecell{4.29\\(3.51)} & \makecell{3.13\\(2.41)} \\
         \midrule
             \multirow{7}{*}{Local} &      Train & \makecell{85.19\\(18.79)} &  \makecell{80.42\\(26.98)} & \makecell{91.75\\(8.21)} &  \makecell{88.0\\(7.93)} &  \makecell{90.95\\(8.0)} & \makecell{85.21\\(9.43)} &       \makecell{3.86\\(3.6)} &  \makecell{5.98\\(7.27)} & \makecell{4.12\\(4.09)} \\
              & Validation & \makecell{80.45\\(20.88)} &  \makecell{62.89\\(33.46)} &  \makecell{89.07\\(8.9)} &  \makecell{90.8\\(7.08)} & \makecell{89.65\\(8.21)} & \makecell{85.14\\(9.38)} &      \makecell{2.68\\(2.69)} &   \makecell{4.94\\(6.1)} & \makecell{3.52\\(3.19)} \\
              &    Holdout &  \makecell{86.41\\(17.5)} &  \makecell{78.35\\(27.47)} & \makecell{91.52\\(8.01)} &  \makecell{89.37\\(7.6)} &  \makecell{91.2\\(7.71)} &  \makecell{85.01\\(9.6)} &      \makecell{2.76\\(2.76)} &  \makecell{6.36\\(7.27)} & \makecell{3.94\\(3.97)} \\
              &       Test & \makecell{68.52\\(30.98)} &   \makecell{61.08\\(34.2)} & \makecell{88.61\\(9.19)} & \makecell{88.13\\(7.81)} & \makecell{88.77\\(8.51)} & \makecell{89.05\\(7.49)} &      \makecell{2.28\\(2.62)} &  \makecell{3.46\\(3.28)} & \makecell{2.48\\(2.11)} \\
              \midrule
            \multirow{7}{*}{Global} &      Train & \makecell{91.86\\(11.95)} &  \makecell{75.19\\(27.65)} & \makecell{91.43\\(8.26)} &  \makecell{87.85\\(7.9)} & \makecell{90.69\\(8.01)} & \makecell{85.34\\(9.22)} &       \makecell{3.73\\(3.9)} &  \makecell{5.55\\(6.55)} & \makecell{3.85\\(3.87)} \\
             & Validation & \makecell{92.29\\(13.52)} &  \makecell{61.85\\(29.62)} & \makecell{89.17\\(8.28)} & \makecell{90.13\\(7.42)} & \makecell{89.51\\(7.95)} &  \makecell{84.91\\(9.8)} &      \makecell{1.96\\(1.89)} &  \makecell{5.19\\(6.77)} & \makecell{3.33\\(3.48)} \\
             &    Holdout & \makecell{87.36\\(23.97)} &  \makecell{75.85\\(26.96)} & \makecell{90.99\\(8.93)} & \makecell{88.78\\(7.87)} & \makecell{90.83\\(8.02)} & \makecell{85.48\\(9.18)} &      \makecell{3.08\\(2.75)} &  \makecell{5.49\\(6.39)} & \makecell{3.67\\(3.47)} \\
             &       Test &  \makecell{85.0\\(21.18)} &   \makecell{62.13\\(32.4)} & \makecell{89.37\\(8.82)} & \makecell{88.26\\(8.03)} & \makecell{89.24\\(8.46)} & \makecell{87.69\\(8.17)} &      \makecell{2.24\\(3.15)} &    \makecell{3.4\\(4.4)} & \makecell{2.42\\(2.74)} \\
\bottomrule
\end{tabular}
}
\caption{Single Sets Results}
\label{tab:single_sets}

\end{table}


==> tables/statistical_low_complexity.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{llllllllllllllllllllr}
\toprule
       &        & \multicolumn{6}{l}{Individual} & \multicolumn{6}{l}{Local} & \multicolumn{6}{l}{Global} &  Summary \\
       &        &              TTVH &             TTVHN &              THT &              THTN &             TTVHT &            TTVHTN &              TTVH &             TTVHN &               THT &              THTN &             TTVHT &            TTVHTN &              TTVH &             TTVHN &               THT &              THTN &             TTVHT &            TTVHTN & Test Acc \\
\midrule
Individual & TTVH &          $\equiv$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &       -6 \\
       & TTVHN &   $\triangledown$ &          $\equiv$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &      -15 \\
       & THT &  $\blacktriangle$ &  $\blacktriangle$ &         $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &       17 \\
       & THTN &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &        7 \\
       & TTVHT &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &       14 \\
       & TTVHTN &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &        2 \\
Local & TTVH &          $\equiv$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &       -6 \\
       & TTVHN &   $\triangledown$ &          $\equiv$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &      -15 \\
       & THT &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &       14 \\
       & THTN &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &        2 \\
       & TTVHT &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &       11 \\
       & TTVHTN &          $\equiv$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &       -3 \\
Global & TTVH &          $\equiv$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &       -7 \\
       & TTVHN &   $\triangledown$ &          $\equiv$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &      -15 \\
       & THT &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &        8 \\
       & THTN &          $\equiv$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &       -8 \\
       & TTVHT &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &        6 \\
       & TTVHTN &          $\equiv$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &       -6 \\
\bottomrule
\end{tabular}
}
\caption{Wilcoxon Statistical Low Complexity Test Accuracy}
\label{tab:statistical_low_complexity}
\end{table}


==> tables/statistical_low_complexity_disagreement_all.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{llllllllllllllllllllr}
\toprule
       &        & \multicolumn{6}{l}{Individual} & \multicolumn{6}{l}{Local} & \multicolumn{6}{l}{Global} &          Summary \\
       &        &             TTVH &             TTVHN &               THT &              THTN &             TTVHT &            TTVHTN &              TTVH &             TTVHN &               THT &              THTN &             TTVHT &            TTVHTN &              TTVH &             TTVHN &               THT &              THTN &             TTVHT &            TTVHTN & All Disagreement $\downarrow$ \\
\midrule
Individual & TTVH &         $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &               17 \\
       & TTVHN &  $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &               11 \\
       & THT &  $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &          $\equiv$ &               -2 \\
       & THTN &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &              -12 \\
       & TTVHT &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &               -9 \\
       & TTVHTN &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &              -13 \\
Local & TTVH &  $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &               13 \\
       & TTVHN &  $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &               10 \\
       & THT &  $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &                3 \\
       & THTN &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &              -11 \\
       & TTVHT &  $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &          $\equiv$ &               -3 \\
       & TTVHTN &  $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &               -9 \\
Global & TTVH &  $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &               12 \\
       & TTVHN &  $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &                2 \\
       & THT &  $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &                7 \\
       & THTN &  $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &               -9 \\
       & TTVHT &  $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &                1 \\
       & TTVHTN &  $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &               -8 \\
\bottomrule
\end{tabular}
}
\caption{Wilcoxon Statistical Significance Test comparisons for Low Complexity policies w.r.t. All Disagreement.}
\label{tab:statistical_low_complexity_disagreement_all}
\end{table}


==> tables/statistical_no_premature_early_stopping.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllllllllllllllllllllllllr}
\toprule
       &         & \multicolumn{9}{l}{Individual} & \multicolumn{9}{l}{Local} & \multicolumn{9}{l}{Global} &  Summary \\
       &         &             TTVHN &            TTVHNB &            TTVHNE &             THTN &             THTNB &             THTNE &            TTVHTN &           TTVHTNE &           TTVHTNB &             TTVHN &            TTVHNB &            TTVHNE &              THTN &             THTNB &             THTNE &            TTVHTN &           TTVHTNE &           TTVHTNB &             TTVHN &            TTVHNB &            TTVHNE &              THTN &             THTNB &             THTNE &            TTVHTN &           TTVHTNE &           TTVHTNB & Test Acc \\
\midrule
Individual & TTVHN &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &       -7 \\
       & TTVHNB &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &      -24 \\
       & TTVHNE &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &       -7 \\
       & THTN &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &         $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &       26 \\
       & THTNB &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &      -12 \\
       & THTNE &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &       18 \\
       & TTVHTN &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &       23 \\
       & TTVHTNE &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &       18 \\
       & TTVHTNB &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &       -6 \\
Local & TTVHN &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &       -6 \\
       & TTVHNB &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &      -24 \\
       & TTVHNE &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &       -6 \\
       & THTN &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &       23 \\
       & THTNB &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &  $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &      -18 \\
       & THTNE &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &       10 \\
       & TTVHTN &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &       18 \\
       & TTVHTNE &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &       11 \\
       & TTVHTNB &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &       -7 \\
Global & TTVHN &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &       -6 \\
       & TTVHNB &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &      -24 \\
       & TTVHNE &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &       -7 \\
       & THTN &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &       10 \\
       & THTNB &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &      -19 \\
       & THTNE &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &        4 \\
       & TTVHTN &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &       13 \\
       & TTVHTNE &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &        6 \\
       & TTVHTNB &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &       -7 \\
\bottomrule
\end{tabular}
}
\caption{Wilcoxon Statistical Early Stopping Test Accuracy}
\label{tab:statistical_no_premature_early_stopping}
\end{table}


==> tables/statistical_similar_sets_performance.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllllllllllllr}
\toprule
       &       & \multicolumn{5}{l}{Individual} & \multicolumn{5}{l}{Local} & \multicolumn{5}{l}{Global} &  Summary \\
       &       &           Holdout &              TTVH &             Test &               THT &             TTVHT &           Holdout &              TTVH &              Test &               THT &             TTVHT &           Holdout &              TTVH &              Test &               THT &             TTVHT & Test Acc \\
\midrule
Individual & Holdout &          $\equiv$ &          $\equiv$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &       -9 \\
       & TTVH &          $\equiv$ &          $\equiv$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &       -8 \\
       & Test &  $\blacktriangle$ &  $\blacktriangle$ &         $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &       14 \\
       & THT &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &       12 \\
       & TTVHT &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &        7 \\
Local & Holdout &          $\equiv$ &   $\triangledown$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &      -10 \\
       & TTVH &          $\equiv$ &          $\equiv$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &       -9 \\
       & Test &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &       10 \\
       & THT &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &        7 \\
       & TTVHT &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &        3 \\
Global & Holdout &          $\equiv$ &          $\equiv$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &       -9 \\
       & TTVH &          $\equiv$ &          $\equiv$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &       -9 \\
       & Test &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &        3 \\
       & THT &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &        0 \\
       & TTVHT &  $\blacktriangle$ &  $\blacktriangle$ &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &       -2 \\
\bottomrule
\end{tabular}
}
\caption{Wilcoxon Statistical Significance Test comparisons between High Robustness policies. $\blacktriangle$: row is significantly better than column, $\equiv$:both are equivalent, and $\triangledown$: row is significantly worse than column. The Summary contains the sum of $\blacktriangle (1)$, $\equiv (0)$, $\triangledown (-1)$ for each policy in rows.}
\label{tab:statistical_similar_sets_performance}
\end{table}


==> tables/statistical_similar_sets_performance_disagreement_all.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllllllllllllr}
\toprule
       &       & \multicolumn{5}{l}{Individual} & \multicolumn{5}{l}{Local} & \multicolumn{5}{l}{Global} &          Summary \\
       &       &          Holdout &              TTVH &              Test &               THT &             TTVHT &           Holdout &              TTVH &              Test &               THT &             TTVHT &           Holdout &              TTVH &              Test &               THT &             TTVHT & All Disagreement \\
\midrule
Individual & Holdout &         $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &               14 \\
       & TTVH &  $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &                9 \\
       & Test &  $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &                6 \\
       & THT &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &               -5 \\
       & TTVHT &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &              -12 \\
Local & Holdout &  $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &                9 \\
       & TTVH &  $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &                5 \\
       & Test &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &              -10 \\
       & THT &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &          $\equiv$ &               -3 \\
       & TTVHT &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &               -7 \\
Global & Holdout &  $\triangledown$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &                8 \\
       & TTVH &  $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &  $\blacktriangle$ &                4 \\
       & Test &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &              -13 \\
       & THT &  $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &  $\blacktriangle$ &                0 \\
       & TTVHT &  $\triangledown$ &   $\triangledown$ &   $\triangledown$ &          $\equiv$ &  $\blacktriangle$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &          $\equiv$ &          $\equiv$ &   $\triangledown$ &   $\triangledown$ &  $\blacktriangle$ &   $\triangledown$ &          $\equiv$ &               -5 \\
\bottomrule
\end{tabular}
}
\caption{Wilcoxon Statistical Significance Test comparisons between High Robustness policies. Since we are analyzing the All Disagreement here, $\blacktriangle$: row is significantly worse than column (larger All Disagreement), $\equiv$: both are equivalent, and $\triangledown$: row is significantly better than column (smaller All Disagreement). The Summary contains the sum of $\blacktriangle (1)$, $\equiv (0)$, $\triangledown (-1)$ for each policy in rows.}
\label{tab:statistical_similar_sets_performance_disagreement_all}
\end{table}

